Computational Asymmetries in Robust Classification

In the context of adversarial robustness, we make three strongly related contributions. First, we prove that while attacking ReLU classifiers is $\mathit{NP}$-hard, ensuring their robustness at training time is $\Sigma^2_P$-hard (even on a single example). This asymmetry provides a rationale for the fact that robust classifications approaches are frequently fooled in the literature. Second, we show that inference-time robustness certificates are not affected by this asymmetry, by introducing a proof-of-concept approach named Counter-Attack (CA). Indeed, CA displays a reversed asymmetry: running the defense is $\mathit{NP}$-hard, while attacking it is $\Sigma_2^P$-hard. Finally, motivated by our previous result, we argue that adversarial attacks can be used in the context of robustness certification, and provide an empirical evaluation of their effectiveness. As a byproduct of this process, we also release UG100, a benchmark dataset for adversarial attacks.

==> app/asymmetries.tex <==
\begin{table}[]
\centering
\caption{Relation between existing defenses and guidelines. Remember that Guideline (1) recommends relying only on the model itself, Guideline (2) imposes that a defense should not be influenced (explicitly or implicitly) by the natural loss, Guideline (3) recommends taking $x$ as a parameter, and Guideline (4) recommends solving a problem with conditions and constraints that are not stricter than those of an attack.}
\begin{tabular}{llllll}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Defense}}} & \multicolumn{4}{c}{\textbf{Follows...}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Broken?}}} \\ \cmidrule{2-5}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{G1}} & \multicolumn{1}{c}{\textbf{G2}} & \multicolumn{1}{c}{\textbf{G3}} & \multicolumn{1}{c}{\textbf{G4 (L)}} & \multicolumn{1}{c}{} \\ \midrule
AAT (detector) \citep{yin2019adversarial} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{No} & No & \citep{tramer2020adaptive} \\
AAT (ensemble) \citep{yin2019adversarial} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{No} & No & \citep{tramer2020adaptive} \\
Adversarial Training \citep{madry2018towards} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (E)} & \multicolumn{1}{l}{No} & No & No \\
Adversarial Retraining \citep{grosse2017statistical} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No} & No & \citep{carlini2017adversarial} \\
APE-GAN \citep{shen2017ape} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{\textasciitilde (H)} & N/A (I) & \citep{carlini2017magnet} \\
Are Generative Classifiers... \citep{li2019generative} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No} & N/A (I) & \citep{tramer2020adaptive} \\
Artifact Detection \citep{feinman2017detecting} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No} & No & \citep{carlini2017adversarial} \\
Attacking Adversarial Attacks \citep{wu2021attacking} & \multicolumn{1}{l}{No (A)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & \citep{croce2022evaluating} \\
Beating Attackers... \citep{wu2020beating} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{Yes} & Yes & No \\
Bounded ReLU \citep{zhang2018efficient} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & \citep{carlini2017magnet} \\
Cascade Adversarial Training \citep{na2017cascade} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (E)} & \multicolumn{1}{l}{No} & No & No \\
Counteracting Adversarial... \citep{zhang2020towards} & \multicolumn{1}{l}{No (A)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & No \\
Defense-GAN \citep{samangouei2018defense} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{\textasciitilde (H)} & N/A (I) & \citep{athalye2018obfuscated} (J) \\
Defensive Distillation \citep{papernot2016distillation} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{No} & N/A (I) & \citep{carlini2016defensive} \\
Defensive Dropout \citep{wang2018defensive} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & \citep{athalye2018obfuscated} (J) \\
Dimensionality Reduction \citep{bhagoji2017dimensionality} & \multicolumn{1}{l}{No (A)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & N/A (I) & \citep{carlini2017adversarial} \\
Dropout Randomization \citep{feinman2017detecting} & \multicolumn{1}{l}{No (A)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{Yes} & Yes & \citep{carlini2017adversarial} (J) \\
EMPIR \citep{sen2020empir} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (E)} & \multicolumn{1}{l}{No} & No & \citep{tramer2020adaptive} \\
Ensemble Diversity \citep{pang2019improving} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (E)} & \multicolumn{1}{l}{No} & No & \citep{tramer2020adaptive} \\
Error Correcting Codes \citep{verma2019error} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{No (E)} & \multicolumn{1}{l}{No} & No & \citep{tramer2020adaptive} \\
Examining Convolutional... \citep{metzen2016detecting} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No} & No & \citep{carlini2017adversarial} (J)\\
Gaussian Data Augmentation \citep{zhang2018efficient} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{No} & N/A (I) & \citep{carlini2017magnet}\\
Hidden Layer PCA \citep{li2017adversarial} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No} & No & \citep{carlini2017adversarial} \\
Input Image PCA \citep{hendrycks2016early} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No} & No & \citep{carlini2017adversarial}\\
Input Transformations \citep{guo2018countering} & \multicolumn{1}{l}{No (A, B)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & \citep{athalye2018obfuscated} \\
k-Winners Take All \citep{xiao2019enhancing} & \multicolumn{1}{l}{No (B)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{No} & Yes & \citep{tramer2020adaptive} \\
Local Intrinsic Dimensionality \citep{ma2018characterizing} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No} & No & \citep{athalye2018obfuscated} \\
MagNet (classifier) \citep{meng2017magnet} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{\textasciitilde (H)} & No & \citep{carlini2017magnet} \\
MagNet (detector) \citep{meng2017magnet} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{\textasciitilde (H)} & N/A (I) & \citep{carlini2017magnet} \\
Maximum Mean Discrepancy \citep{grosse2017statistical} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{No} & \multicolumn{1}{l}{N/A (K)} & No & \citep{carlini2017adversarial} \\
ME-Net \citep{yang2019me} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{\textasciitilde (H)} & N/A (I) & \citep{tramer2020adaptive} \\
Mean Blur \citep{li2017adversarial} & \multicolumn{1}{l}{No (A)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{Yes} & No & \citep{carlini2017adversarial} (J) \\
Mixup Inference \citep{pang2019mixup} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & \citep{tramer2020adaptive} \\
Mitigating Through... \citep{xie2018mitigating} & \multicolumn{1}{l}{No (A, C)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & \citep{athalye2018obfuscated} \\
OOAT \citep{wang2020once} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{Yes (G)} & \multicolumn{1}{l}{No} & No & No \\
PixelDefend \citep{song2017pixeldefend} & \multicolumn{1}{l}{No (B, D)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{\textasciitilde (H)} & N/A (I) & \citep{athalye2018obfuscated} \\ 
Re-Attacking \citep{ahmadi2021adversarial} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{\textasciitilde (H)} & N/A (I) & No \\
Rethinking Softmax.. \citep{pang2019rethinking} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No (E)} & \multicolumn{1}{l}{No} & No & \citep{tramer2020adaptive} \\
RSFT \citep{bafna2018thwarting} & \multicolumn{1}{l}{No (A)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & \citep{tramer2020adaptive} \\
ShieldNets (classifier) \citep{theagarajan2019shieldnets} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{No} & \multicolumn{1}{l}{\textasciitilde (H)} & N/A (I) & No \\
ShieldNets (detector) \citep{theagarajan2019shieldnets} & \multicolumn{1}{l}{No (D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{\textasciitilde (H)} & N/A (I) & No \\
Stochastic Activation Pruning \citep{dhillon2018stochastic} & \multicolumn{1}{l}{No (C)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{Yes} & Yes & \citep{athalye2018obfuscated} \\
The Odds are Odd \citep{roth2019odds} & \multicolumn{1}{l}{No (A, B, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{No} & No & \citep{tramer2020adaptive} \\
Thermometer Encoding \citep{goodfellow2015explaining} & \multicolumn{1}{l}{No (A, B)} & \multicolumn{1}{l}{No (F)} & \multicolumn{1}{l}{No} & Yes & \citep{athalye2018obfuscated}  \\
Turning a Weakness... \citep{hu2019new} & \multicolumn{1}{l}{No (A, D)} & \multicolumn{1}{l}{Yes} & \multicolumn{1}{l}{Yes} & Yes & \citep{tramer2020adaptive} \\
\bottomrule
\end{tabular}
\label{tab:asymmetries}
\end{table}

\begin{table}[]
\caption{Reference for observations in \Cref{tab:asymmetries}.}
\centering
\begin{tabular}{ll}
\toprule
\textbf{Letter} & \multicolumn{1}{c}{\textbf{Observation}} \\ \midrule
A & Assumes or learns properties of adversarial examples \\
B & Relies on the assumption that the attacker does not have full information \\
C & Relies on the assumption that the attacker cannot deal with randomness \\
D & Requires genuine data \\
E & Explicit role of loss \\
F & Implicit loss constraint (effect on loss or accuracy) \\
G & Provides an explicit accuracy-robustness trade-off \\
H & A non-trivial part of the computation is performed before the input is known \\
I & Problem statements are not directly comparable \\
J & Partially broken \\
K & Classifies \emph{sets} of inputs \\
L & Analysis is heavily influenced by what is defined to be the success condition \\
\bottomrule
\end{tabular}
\label{tab:asymmetriesLegend}
\end{table}

==> app/comparison.tex <==
\section{Overview of Certified Defenses}
\label{sec:comparison}

In order to put CA into context, we provide an overview of common approaches to certified robustness, as well as their strengths and weaknesses.

% Structure 1:
% - Bounds
% - Verifiers
% - Specific Threat models
% - Probabilistic Robustness

% Structure 2:
% - Weak bounds
% - Long times
% - Specific Threat models
% - Probabilistic Robustness

Initially, theoretical work focused on providing robustness bounds based on general properties. For example, \citet{szegedy2013intriguing} computed robustness bounds against $L^2$-bounded perturbations by studying the upper Lipschitz constant of each layer, while \citet{hein2017formal} achieved similar results for $L^p$-bounded perturbations by focusing on local Lipschitzness.
While these studies do not require any modifications to the network or distribution hypotheses, in practice the provided bounds are too loose to be used in practice. For this reason, \citet{weng2018evaluating} derived stronger bounds through a local Lipschitz constant estimation technique; however, finding this bound is computationally expensive, which is why the authors also provide a heuristic to estimate it.

% Volendo si può citare anche 

% Put them at the end?
Similarly, solver-based approaches provide tight bounds but require expensive computations. For example, Reluplex was used to verify networks of at most $\sim$300 ReLU nodes \citep{katz2017reluplex}. Later works managed to reduce complexity using alternative formulations \citep{dvijotham2018dual,singh2018fast,tjeng2019evaluating}. In particular,  \citet{tjeng2019evaluating} was able to use a MIP-based formulation to significantly speed up verification, although large networks are still not feasible to verify. Solver-friendly training techniques can boost the performance of verifiers (such as in \citep{xiao2019training} and \citep{leino2021globally}); however, this increase in speed often comes at the cost of accuracy (see \Cref{sec:experimentalSetup}).
% Other solver stuff?

% Restricted threat model
Another solution to the trade-off between speed and bound tightness is to focus on specific (and more tractable) threat models. For example, \citet{han2021scalecert} provide robustness guarantees against adversarial patches \citep{brown2017adversarial}, while \citet{jia2019certified} focus on adversarial word substitutions. In the same vein, \citet{raghunathan2018certified} provide robustness bounds for specific architectures (i.e. 1-layer and 2-layer neural networks), while \citet{zhang2021towards} introduce custom neurons that, if used in place of regular neurons, provide $L^\infty$ robustness guarantees. These techniques thus trade generality for speed.

The most common approach, however, consists in providing statistical guarantees. For example, \citet{sinha2018certifying} showed that using a custom loss can bound the adversarial risk. Similarly, \citet{dan2020sharp} proved adversarial risk bounds for Gaussian mixture models depending on the "adversarial Signal-to-Noise Ratio". Finally, \citet{cohen2019certified} introduced a smoothing-based certified defense that, due to its high computational cost, is replaced by a Monte Carlo estimate with a given probability of being robust. This work was later expanded upon in \citep{salman2020denoised} and \citep{carlini2022certified}.
The main drawback of these techniques is the fact that they cannot be used in contexts where statistical guarantees are not sufficient, such as safety-critical applications.

All of these certified defenses prioritize certain aspects (speed, strength, generality) over others.
In the context of this (simplified) framework, CA in its exact form can be thus considered a defense that prioritizes strength and generality over speed, similarly to \citet{katz2017reluplex} and \citet{tjeng2019evaluating}.

%Of all defenses, CA can be thus considered

% Table with pros and cons?
% Summary table


==> app/fooling.tex <==
\section{Results for Attacks against CA}
\label{app:fooling}

We report the parameters for the variant of our attack in \Cref{tab:ccaParameters}, while we report its success rate in \Cref{tab:foolingResults}. We set $\varepsilon = \varepsilon^\prime$ equal to $\{0.025, 0.05, 0.1\}$ for MNIST and $\{2/255, 4/255, 8/255\}$ for CIFAR10. Note that, since Deepfool is a deterministic attack, no measures against randomizations were taken.

\begin{table}[]
\caption{Parameters for the variant of the PGD attack.}
\centering
\begin{tabular}{ll}
\toprule
\textbf{Parameter} & \textbf{Value} \\\midrule
$\lambda$ & $\{10^{-4}, 10^{-2}, 1, 10^{2}, 10^4\}$ \\ \midrule
NES Estimation Samples & 200 \\ \midrule
NES Estimation $\varepsilon$ & $10^{-4}$ \\ \midrule
PGD Iterations & 400 \\ \midrule
PGD $\varepsilon$ & $10^{-3}$ \\
\bottomrule
\end{tabular}
\label{tab:ccaParameters}
\end{table}


\begin{table}[]
\centering
\caption{Success rate of the pool composed of the anti-CA variant of PGD and uniform noise for the A architectures.}
\begin{subtable}[]{0.5\textwidth}
\centering
\begin{tabular}{lllll}
\toprule
\multirow{2}{*}{$\varepsilon$} & \multicolumn{4}{c}{\textbf{$\varepsilon^\prime$ Multiplier}} \\ \cmidrule{2-5} 
 & \textbf{1x} & \textbf{2x} & \textbf{5x} & \textbf{10x} \\ \midrule
0.025 & 0\% & 23\% & 95\% & 100\% \\ \midrule
0.05 & 3\% & 41\% & 97\% & 100\% \\ \midrule
0.1 & 2\% & 50\% & 96\% & 100\% \\ \bottomrule
\end{tabular}
\caption{MNIST A Standard}
\end{subtable}%
\begin{subtable}[]{0.5\textwidth}
\centering
\begin{tabular}{lllll}
\toprule
\multirow{2}{*}{$\varepsilon$} & \multicolumn{4}{c}{\textbf{$\varepsilon^\prime$ Multiplier}} \\ \cmidrule{2-5} 
 & \textbf{1x} & \textbf{2x} & \textbf{5x} & \textbf{10x} \\ \midrule
2/255 & 0\% & 34\% & 96\% & 100\% \\ \midrule
4/255 & 1\% & 50\% & 100\% & 100\% \\ \midrule
8/255 & 1\% & 58\% & 100\% & 100\% \\ \bottomrule
\end{tabular}
\caption{CIFAR10 A Standard}
\end{subtable}

\label{tab:foolingResults}
\end{table}




==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf -shell-escape \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
